Efficient Personalized Text-to-image Generation by Leveraging Textual Subspace

Personalized text-to-image generation has attracted unprecedented attention in the recent few years due to its unique capability of generating highly-personalized images via using the input concept dataset and novel textual prompt. However, previous methods solely focus on the performance of the reconstruction task, degrading its ability to combine with different textual prompt. Besides, optimizing in the high-dimensional embedding space usually leads to unnecessary time-consuming training process and slow convergence. To address these issues, we propose an efficient method to explore the target embedding in a textual subspace, drawing inspiration from the self-expressiveness property. Additionally, we propose an efficient selection strategy for determining the basis vectors of the textual subspace. The experimental evaluations demonstrate that the learned embedding can not only faithfully reconstruct input image, but also significantly improves its alignment with novel input textual prompt. Furthermore, we observe that optimizing in the textual subspace leads to an significant improvement of the robustness to the initial word, relaxing the constraint that requires users to input the most relevant initial word. Our method opens the door to more efficient representation learning for personalized text-to-image generation.

==> algorithm3.tex <==
\begin{algorithm}[ht!]
\caption{Algorithm of Sparse Sub-representation.}
\label{alg:method3}
\begin{algorithmic}
   \STATE {\bfseries Input:} 
   Input Image Dataset $\mathcal{D}$, Pre-trained Diffusion Network $u_\theta$, Reconstruction Objective $\mathscr{L}_{rec}$, Pre-defined Vocabulary Matrix $V$, Dimension of the Embedding Space $d$, Weight Threshold $\epsilon_{thr}$, Initialization embedding $v^{i_0}$, Dimension Threshold $d_{thr}$, Weight Vector $w_{i_0}$, Training Iteration $n_1$, Input Prompt $S$
   \STATE {\bfseries Phase 1: Searching Sparse Sub-representation}
   \STATE Solve constrained optimization $\min \Vert w_{i_0} \Vert_1$, \text{s.t.}, $v^{i_0}=Vw_{i_0}$, $w_{i_0, i_0}=0$
   \STATE Output sparse weight vector $w_{i_0}'$
   \STATE {\bfseries Phase 2: Candidate Selection}
   \STATE Select candidate embeddings $\{v_{can}^i\}_{i=1}^M$ such that each weight $|w_{can}'| > \epsilon_{thr}$
   \STATE {\bfseries Phase 3: Training by Updating Weights}
   \FOR{$i=1$ {\bfseries to} $n_1$}
   \STATE Sample  a minibatch $\{ \boldsymbol{x}\} \sim \mathcal{D}$ 
   \STATE Update embeddings $\{w_i\}_{i=1}^M \leftarrow \nabla_{(w_1,\dots,w_M)}\mathscr{L}_{rec}(\{ \boldsymbol{x}\}, \{w_i\}_{i=1}^M)$
   \ENDFOR
   \STATE Get trained weights of the candidate embeddings $\{w_{i}^*\}_{i=1}^M$
   \STATE Obtain learned embedding using linear combination $v_* \leftarrow \sum_{i=0}^M w_{i}^* v_{can}^i$
   \STATE {\bfseries Phase 3: Multi-concept Generation with Learned Embeddings}
   \STATE Combine learned embeddings with input prompt $S_* \leftarrow \textit{Combine}(S, v_*)$
   \STATE Get target images through pretrained diffusion model $y \leftarrow u_\theta(S_*)$
   \STATE {\bfseries Output:} Target images: $y$
   \end{algorithmic}
\end{algorithm}

==> dimension-and-distance-effect.tex <==
\begin{figure}[htbp]
\centering

\begin{comment}
\begin{minipage}[t]{0.49\textwidth}
\label{fig:dimension-effect}
\includegraphics[width=0.99\columnwidth]{figure/dimension-effect.pdf}
\caption{Dimension of textual subspace.}
\end{minipage}
\begin{minipage}[t]{0.49\textwidth}
\label{fig:distance-effect}
\includegraphics[width=0.99\columnwidth]{figure/distance-effect.pdf}
\caption{Distance measurement.}
\end{minipage}
\end{comment}

\subfigure[Dimension of textual subspace]{
\label{fig:dimension-effect}
\includegraphics[width=0.99\columnwidth]{figure/dimension-effect.pdf}
}
\subfigure[Distance measurement]{
\label{fig:distance-effect}
\includegraphics[width=0.99\columnwidth]{figure/distance-effect.pdf}
}

\caption{Comparison about effect of dimension of the textual subspace.}
\label{fig:dimension-and-distance-effect}
\end{figure}

==> dimension-effect.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.99\linewidth]{figure/dimension-effect.pdf}
\caption{Comparison about effect of dimension of the textual subspace.}
\label{fig:dimension-effect}
\end{figure}

==> distance-and-tabular.tex <==
\begin{figure*}[htbp]
\begin{minipage}[b]{0.48\linewidth}
\centering
% \resizebox{1.0\linewidth}{!}{
\includegraphics[width=\linewidth]{figure/distance-effect.png}
% }
%\vspace{-0.2in} 
\caption{Comparison about text-image alignment score of different type of vector distance with respect to training steps.}
\label{fig:distance-effect}
%\vspace{-0.1in}
\end{minipage}
\hspace{0.05in}
\begin{minipage}[b]{0.48\linewidth}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{|c|}{\textbf{Text}} & \multicolumn{2}{|c|}{\textbf{Image}} \\
\cline{2-5}
& ``cat'' & ``animal'' & ``cat'' & ``animal'' \\
\midrule
Dreambooth & 0.74 & 0.63 & 0.91 & 0.91 \\
\hline
Custom-Diffusion & 0.79 & 0.69 & 0.87 & 0.82 \\
\hline
Textual Inversion & 0.62 & 0.62 & 0.89 & 0.86 \\
\hline
BaTex (ours) & 0.76 & 0.75 & 0.88 & 0.88 \\
\bottomrule
\end{tabular}
}
\captionof{table}{Comparison of BaTex and three previous works about the robustness against initial word. We take the \textit{Cat} dataset as an example and use ``animal'' to replace the original initial word ``cat''.}
\label{tab:initialization-effect}
\end{minipage}
\vspace{-0.2in}
\end{figure*}

==> quantitative-comparison-new.tex <==
\begin{table}[htbp]
\centering
\small
\begin{tabular}{ccc|cccccc}
\toprule
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Metric}} & Cat & Wooden-pot & Gta5-artwork  & Anders-zorn & Cute-game & \multirow{2}{*}{\textbf{Mean}} \\
& & & [5] & [4] & [14] & [12] & [8] & \\
\midrule
& \multirow{2}{*}{Dreambooth} & Text & 0.74 (0.00) & 0.63 (0.01) & 0.72 (0.01) & 0.72 (0.01) & 0.62 (0.00) & 0.69 \\
Model & & Image & 
\textcolor{red}{0.91 (0.01)} & \textcolor{red}{0.88 (0.01)} & 0.61 (0.01) & \textcolor{red}{0.74 (0.00)} & 0.61 (0.01) & \textcolor{red}{0.75} \\ 
\cline{2-9}
Optimization & \multirow{2}{*}{Custom Diffusion} & Text & \textcolor{red}{0.79 (0.00)} & \textcolor{blue}{0.71 (0.00)} & \textcolor{blue}{0.74 (0.01)} & \textcolor{blue}{0.74 (0.01)} & \textcolor{blue}{0.74 (0.00)} & \textcolor{blue}{0.74} \\ 
& & Image & 0.87 (0.00) & 0.75 (0.00) & 0.59 (0.01) & 0.60 (0.02) & 0.56 (0.00) & 0.68 \\ 
\hline
& \multirow{2}{*}{Textual Inversion} & Text & 0.62 (0.00) & 0.66 (0.01) & 0.78 (0.01) & 0.72 (0.01) & 0.72 (0.00) & 0.70 \\
Embedding & & Image & \textcolor{blue}{0.89 (0.01)} & \textcolor{blue}{0.81 (0.00)} & \textcolor{red}{0.67 (0.01)} & 0.67 (0.01) & \textcolor{red}{0.68 (0.01)} & \textcolor{blue}{0.74} \\
\cline{2-9}
Optimization & \multirow{2}{*}{BaTex (ours)} & Text &  \textcolor{blue}{0.76 (0.00)} & \textcolor{red}{0.72 (0.01)} & \textcolor{red}{0.80 (0.00)} & \textcolor{red}{0.77 (0.00)} & \textcolor{red}{0.77 (0.01)} & \textcolor{red}{0.76} \\
& & Image & 0.88 (0.01) & \textcolor{blue}{0.81 (0.01)} & \textcolor{blue}{0.66 (0.01)} & \textcolor{blue}{0.72 (0.00)} & \textcolor{blue}{0.66 (0.01)} & \textcolor{blue}{0.74} \\
\bottomrule
\end{tabular}
\caption{Quantitative comparison between BaTex and previous works. The numbers in square bracket and parenthesis are the number of image in the dataset and the standard deviation. ``Text'' and ``Image'' refer to text-image and image-image alignment scores respectively. Red and blue indicate the best and second best results respectively. While our method achieves similar results to Textual Inversion in terms of image reconstruction, we significantly outperform them in terms of text similarity, and even achieve results comparable to the methods of the ``Model Optimization'' category. The results are reported with standard deviation over five random seeds.}
\label{tab:quantitative-comparison-new}
\end{table}

==> second-effect.tex <==
\begin{figure}[htbp]
\label{fig:second-effect}
\centering

\includegraphics[width=0.99\linewidth]{figure/second-effect.pdf}

\caption{Effect of adding additional intialization word.}
\end{figure}

==> step-effect.tex <==
\begin{figure}[htbp]
\label{fig:step-effect}
\centering

\includegraphics[width=0.99\linewidth]{figure/step-effect.pdf}

\caption{Text and image alignment scores with respect to training steps. To show the reason for our choice of training steps, we plot the results recording every 50 steps for the first 1000 steps, showing that our model reaches convergence at about \textbf{500} steps.}
\end{figure}

==> tabular-multi-concept.tex <==
\begin{sidewaystable}[thp]
\label{tab:multi-concept}
\begin{center}
\begin{tabular}
{ccc|ccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Metrics}} & \multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Models}} & Cat & Chair & Dog  & Barn & Teddybear & Flower & Physics Mug & Elephant & Style1  & Style2 & \textbf{Mean} \\
& & & (5) & (4) & (10) & (7) & (7) & (10) & (5) & (5) & (a) & (b) & \textbf{(std)} \\
\midrule
& \multirow{2}{*}{Model} & Dream- & \multirow{2}{*}{a1} & \multirow{2}{*}{a2} & \multirow{2}{*}{a3} & \multirow{2}{*}{a4} & \multirow{2}{*}{a5} & \multirow{2}{*}{a6} & \multirow{2}{*}{a7} & \multirow{2}{*}{a8} & \multirow{2}{*}{a9} & \multirow{2}{*}{a10} & \multirow{2}{*}{a11} \\
& & Booth & & & & & & & & & & & \\
\cline{3-14}
\multirow{2}{*}{Text} & \multirow{2}{*}{optimization} & Custom- & \multirow{2}{*}{a1} & \multirow{2}{*}{a2} & \multirow{2}{*}{a3} & \multirow{2}{*}{a4} & \multirow{2}{*}{a5} & \multirow{2}{*}{a6} & \multirow{2}{*}{a7} & \multirow{2}{*}{a8} & \multirow{2}{*}{a9} & \multirow{2}{*}{a10} & \multirow{2}{*}{a11} \\
& & Diffusion & & & & & & & & & & & \\
\cline{2-14}
\multirow{2}{*}{alignment} & \multirow{2}{*}{Embedding} & Textual & \multirow{2}{*}{a1} & \multirow{2}{*}{a2} & \multirow{2}{*}{a3} & \multirow{2}{*}{a4} & \multirow{2}{*}{a5} & \multirow{2}{*}{a6} & \multirow{2}{*}{a7} & \multirow{2}{*}{a8} & \multirow{2}{*}{a9} & \multirow{2}{*}{a10} & \multirow{2}{*}{a11} \\
& & Inversion & & & & & & & & & & & \\
\cline{3-14}
& \multirow{2}{*}{optimization} & \multirow{2}{*}{Ours} & \multirow{2}{*}{a1} & \multirow{2}{*}{a2} & \multirow{2}{*}{a3} & \multirow{2}{*}{a4} & \multirow{2}{*}{a5} & \multirow{2}{*}{a6} & \multirow{2}{*}{a7} & \multirow{2}{*}{a8} & \multirow{2}{*}{a9} & \multirow{2}{*}{a10} & \multirow{2}{*}{a11} \\
& & & & & & & & & & & & & \\
\hline
& \multirow{2}{*}{Model} & Dream- & \multirow{2}{*}{a1} & \multirow{2}{*}{a2} & \multirow{2}{*}{a3} & \multirow{2}{*}{a4} & \multirow{2}{*}{a5} & \multirow{2}{*}{a6} & \multirow{2}{*}{a7} & \multirow{2}{*}{a8} & \multirow{2}{*}{a9} & \multirow{2}{*}{a10} & \multirow{2}{*}{a11} \\
& & Booth & & & & & & & & & & & \\
\cline{3-14}
\multirow{2}{*}{Image} & \multirow{2}{*}{optimization} & Custom- & \multirow{2}{*}{a1} & \multirow{2}{*}{a2} & \multirow{2}{*}{a3} & \multirow{2}{*}{a4} & \multirow{2}{*}{a5} & \multirow{2}{*}{a6} & \multirow{2}{*}{a7} & \multirow{2}{*}{a8} & \multirow{2}{*}{a9} & \multirow{2}{*}{a10} & \multirow{2}{*}{a11} \\
& & Diffusion & & & & & & & & & & & \\
\cline{2-14}
\multirow{2}{*}{alignment} & \multirow{2}{*}{Embedding} & Textual & \multirow{2}{*}{a1} & \multirow{2}{*}{a2} & \multirow{2}{*}{a3} & \multirow{2}{*}{a4} & \multirow{2}{*}{a5} & \multirow{2}{*}{a6} & \multirow{2}{*}{a7} & \multirow{2}{*}{a8} & \multirow{2}{*}{a9} & \multirow{2}{*}{a10} & \multirow{2}{*}{a11} \\
& & Inversion & & & & & & & & & & & \\
\cline{3-14}
& \multirow{2}{*}{optimization} & \multirow{2}{*}{Ours} & \multirow{2}{*}{a1} & \multirow{2}{*}{a2} & \multirow{2}{*}{a3} & \multirow{2}{*}{a4} & \multirow{2}{*}{a5} & \multirow{2}{*}{a6} & \multirow{2}{*}{a7} & \multirow{2}{*}{a8} & \multirow{2}{*}{a9} & \multirow{2}{*}{a10} & \multirow{2}{*}{a11} \\
& & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\end{center}
\caption{Quantitative comparisons on multi-concept generation. ``Model optimization'' and ``Embedding optimization'' refer to methods optimizing pretrained model parameters and word embedding respectively. While ``Model optimization'' methods often have better performance at the cost of overfitting, our method achieves state-of-the-art results in the category of ``Embedding optimization'' and is comparable with ``Model optimization'' methods without overfitting or introducing another regularization dataset. The results are reported with standard deviation over five random seeds.}
\end{sidewaystable}

==> time-comparison.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|ccc}
\toprule
\textbf{Stage} & Textual Inversion & Selection Strategy & BaTex (Ours) \\
\midrule
Time Usage (s) & $3705.3$ & $0.2$ & $495.0$ \\
\bottomrule
\end{tabular}
\caption{Time comparison of each stage of our method and baseline.}
\label{tab:time-comparison}
\end{table}

==> top-number-similar.tex <==
\begin{figure}[t]
    \begin{minipage}[b]{0.5\linewidth}
    \centering
    \subfloat[][Qualitative results using the top one vector.]{\label{fig:top-one}\includegraphics[width=0.99\linewidth]{figure/top-one-teddybear.pdf}}
    \quad
    \subfloat[][Qualitative results using two similar concepts.]{\label{fig:similar-objects}\includegraphics[width=0.99\linewidth]{figure/similar-objects-new.pdf}}
    \end{minipage}
    \medskip
    \begin{minipage}[b]{0.5\linewidth}
    \centering
    \subfloat[][Qualitative comparison of the number of reference images using the \textit{Dog} dataset.]{\label{fig:number-comparison}\includegraphics[width=0.75\linewidth]{figure/number-comparison-dog.pdf}}
    \end{minipage}
    \label{fig:top-number-similar}
\end{figure}
